Privacy Requirements and Realities of Digital Public Goods

In the international development community, the term "digital public goods" is used to describe open-source digital products (e.g., software, datasets) that aim to address the United Nations (UN) Sustainable Development Goals. DPGs are increasingly being used to deliver government services around the world (e.g., ID management, healthcare registration). Because DPGs may handle sensitive data, the UN has established user privacy as a first-order requirement for DPGs. The privacy risks of DPGs are currently managed in part by the DPG standard, which includes a prerequisite questionnaire with questions designed to evaluate a DPG's privacy posture. This study examines the effectiveness of the current DPG standard for ensuring adequate privacy protections. We present a systematic assessment of responses from DPGs regarding their protections of users' privacy. We also present in-depth case studies from three widely-used DPGs to identify privacy threats and compare this to their responses to the DPG standard. Our findings reveal limitations in the current DPG standard's evaluation approach. We conclude by presenting preliminary recommendations and suggestions for strengthening the DPG standard as it relates to privacy. Additionally, we hope this study encourages more usable privacy research on communicating privacy, not only to end users but also third-party adopters of user-facing technologies.

==> related_work.tex <==
\AM{
[Factors that influence contributions to DPGs] \cite{chen2023motivating} checks how to get experts to contribute to DPGs (e.g., Wikipedia). We can probably get the definition of a DPG from this paper, and see what the advantages are of improving the quality of DPGs (which our study wants to do through improving the evaluation process). 
}

\AM{
[DPG governance, case studies] \cite{eaves2022best} conducts an interview study + literature review + DPG case studies to find out governance best practices that DPGs should undertake (Codifying a Vision, Mission, and Values Statement; Creating a Code of Conduct; Designing Governance Bodies; Ensuring Stakeholder Voice and Representation; and Engaging External Contributors. Most relevant recommendations for us: Designing Governance Bodies (however I think this refers to a DPG internal body, not DPGA). We can also look at their literature review (especially Governance in Open Source). 
}

\AM{
[DPG governance] \cite{gillwald2019governance} proposes a "typology of global governance of DPGs". They consider the Internet as a DPG (please check this). Identifies gaps in the current approach. Proposes a multi-stakeholder approach (like us). 
}

\AM{
[Factors that influence contributions to DPGs] \cite{kummer2020unemployment} shows "how individuals engage in socially useful activities after an increase in unemployment." The socially useful activity -> contributing to DPGs (e.g., Wikipedia).
}

\AM{
[DPG outcomes, case studies] \cite{mukherjee2021fast} describes case studies to "explain the concept of digital building blocks as public goods and
how it applies to developmental challenges—poverty, inequality, health, education, public administration, and governance — that span entire populations".
}

\AM{
[DPG outcomes] \cite{nicholson2022agenda} tries to answer the question 'How can DPGs contribute to sustainable development and what are the underlying challenges and opportunities to achieve the Sustainable Development Goals?'. They 'identify five core areas where more research is needed to understand DPGs as a particular type of digital technology and with certain traits of openness'. 'Whether the DPG will ‘do harm’ or not is not an attribute of the technology alone, but a consequence of how it is implemented and used and may change over time.'
}

\AM{
[case studies] \cite{nicholson2022digital} 
}

\AM{
\cite{saebo2021digital}
}

\AM{
\cite{sturmer2023digital}
}

\AM{
\cite{tavares2023digital}
}
